Refinement Reflection (or, how to turn your favorite language into a proof assistant using SMT)

Refinement Reflection turns your favorite programming language into a proof assistant by reflecting the code implementing a user-defined function into the function's (output) refinement type. As a consequence, at uses of the function, the function definition is unfolded into the refinement logic in a precise, predictable and most importantly, programmer controllable way. In the logic, we encode functions and lambdas using uninterpreted symbols preserving SMT-based decidable verification. In the language, we provide a library of combinators that lets programmers compose proofs from basic refinements and function definitions. We have implemented our approach in the Liquid Haskell system, thereby converting Haskell into an interactive proof assistant, that we used to verify a variety of properties ranging from arithmetic properties of higher order, recursive functions to the Monoid, Applicative, Functor and Monad type class laws for a variety of instances.

==> ackermann.tex <==
\begin{figure}
\textbf{Definition}
\[
\begin{array}{lr}
\ack{n}{x}
 \left\{
\begin{array}{l}
\setlength\arraycolsep{0pt}
\begin{array}{ll}
      x+2 &\quad \text{, if}\ n=0 \\
      2   &\quad \text{, if}\ x=0 \\
\end{array} \\
\ack{n-1}{\ack{n}{x-1}}
\end{array}
\right.
&
\iack{h}{n}{x}
 \left\{
\begin{array}{l}
      x \quad \text{, if}\ h=0 \\
      \ack{n}{\iack{h-1}{n}{x}}
\end{array}
\right.
\end{array}
 \]

\textbf{Properties}
$$
\begin{array}{lrcrcl}
1.&                &&            \ack{n+1}{x}   &=& \iack{x}{n}{2}\\
2.&                &&            x + 1          &<& \ack{n}{x}\\
3.&                &&            \ack{n}{x}     &<& \ack{n}{x+1}\\
4.& x < y          &\Rightarrow& \ack{n}{x}     &<& \ack{n}{y}\\
5.& 0 < x          &\Rightarrow& \ack{n}{x}     &<& \ack{n+1}{x}\\
6.& 0 < x, n < m   &\Rightarrow& \ack{n}{x}     &<& \ack{m}{x}\\
7.&                &&            \iack{h}{n}{x} &<& \iack{h+1}{n}{x}\\
8.&                &&            \iack{h}{n}{x} &<& \iack{h}{n}{x+1}\\
9.& x<y            &\Rightarrow& \iack{h}{n}{x} &<& \iack{h}{n}{y}\\
10.&               &\Rightarrow& \iack{h}{n}{x} &<& \iack{h}{n+1}{x}\\
11.& 0<n, l-2 < x  &\Rightarrow& x + l          &<& \ack{n}{x}\\
12.& 0<n, l-2 < x  &\Rightarrow& \iack{l}{n}{x} &<& \ack{n+1}{x}\\
13.&               &&            \iack{x}{n}{y} &<& \ack{n+1}{x+y}\\
\end{array}
$$
\caption{Ackermann Properties~\citep{ackermann}, $\forall n, m, x, y, h, l \geq 0$}
\label{fig:ackermann}
\end{figure}


==> defunctionalization.tex <==



Initial environment: Sort

$$
\begin{array}{rrcl}
\emphbf{SMT Sorts} \quad 
  & \sort
  & ::=   & \tint \spmid \tbool \spmid \tuniv \spmid \tsmtfun{\sort}{\sort}
\\[0.05in]
\end{array}
$$

Free Variables-Initial Environment $\smtenv_I$
\begin{align*}
\text{uvar}_c&:\embed{\constty{c}}, \text{for every functional constant}\ c \\
\dc&:\embed{\constty{c}}, \text{for every data constructor}\ \dc\\
\smtappname{\sort_x}{\sort}&: \tsmtfun{\sort_x}{\sort} \rightarrow \sort_x \rightarrow \sort , 
\text{for every SMT sorts}\ \sort, \sort_x\\
\selector{\dc}{i} &: \embed{\constty{\dc} \rightarrow \typ_i}, 
\text{with}\ \constty{\dc} = \typ_1 \rightarrow \dots \rightarrow \typ_n\rightarrow\typ\\
& \text{for every data con}\ \dc\ \text{with arity}\ i
\end{align*}




Embedding of Types
\begin{align*}
\embed{\tint} &=\tint\\
\embed{\tbool} &=\tbool\\
\embed{T}     &= \tuniv\\
\embed{\tfunbasic{x}{\typ_x}{\typ}} &= \tsmtfun{\embed{\typ_x}}{\embed{\typ}}
\end{align*}


Embedding of Environments
\begin{align*}
\embed{\emptyset} &= \emptyset \\
\embed{\env, \tbind{x}{\typ}} &= \embed{\env}, \tbind{x}{\embed{\typ}}
\end{align*}

\NV{What happens with polymorphic functions?}



\begin{align*}
\smtapp{\tsmtfun{\sort_x}{\sort}}{p_f}{p_x} 
   = \smtappname{\sort_x}{\sort}\ {p_f}\ p_x
\end{align*}




\emphbf{Defunctionalization}\hfill{\tologic{\Gamma}{e}{\typ}{p}{\sort}{\smtenv}{\axioms}}
$$
\inference{
}{
	\tologic{\env}{\etrue}{\tbool}{\etrue}{\tbool}{\emptyset}{\etrue}
}[\lgtrue]
$$
$$
\inference{
}{
	\tologic{\env}{\efalse}{\tbool}{\efalse}{\tbool}{\emptyset}{\etrue}
}[\lgfalse]
$$
$$
\inference{
}{
	\tologic{\env}{n}{\tint}{n}{\tint}{\emptyset}{\etrue}
}[\lgint]
$$

Binary operators
$$
\inference{
    \tologic{\env}{e_1}{\typ}{p_1}{\embed{\typ}}{\smtenv}{\axioms_1} \\
    \tologic{\env}{e_1}{\typ}{p_1}{\embed{\typ}}{\smtenv}{\axioms_2}
}{
	\tologic{\env}{e_1 = e_2}{\tbool}{p_1 = p_2}{\tbool}{\smtenv}{\axioms_1\land \axioms_2}  
}[\lgbinEQ]
$$
$$
\inference{
    \tologic{\env}{e_1}{\tint}{p_1}{\tint}{\smtenv}{\axioms_1} \\
    \tologic{\env}{e_1}{\tint}{p_1}{\tint}{\smtenv}{\axioms_2}
}{
	\tologic{\env}{e_1 < e_2}{\tbool}{p_1 < p_2}{\tbool}{\smtenv}{\axioms_1\land \axioms_2}  
}[\lgbinINT]
$$
$$
\inference{
    \tologic{\env}{e_1}{\tbool}{p_1}{\tbool}{\smtenv}{\axioms_1} \\ 
    \tologic{\env}{e_1}{\tbool}{p_1}{\tbool}{\smtenv}{\axioms_2}
}{
	\tologic{\env}{e_1 \land e_2}{\tbool}{p_1 \land p_2}{\tbool}{\smtenv}{\axioms_1\land \axioms_2}  
}[\lgbinBOOL]
$$

$$
\inference{
    \tologic{\env}{e_1}{\typ}{p_1}{\embed{\typ}}{\smtenv}{\axioms_1} \\
    \tologic{\env}{e_1}{\typ}{p_1}{\embed{\typ}}{\smtenv}{\axioms_2}
}{
	\tologic{\env}{\odot\ e_1 \ e_2}{\tbool}{\odot\ p_1 \ p_2}{\tbool}{\smtenv}{\axioms_1\land \axioms_2}  
}[\lgbinGEN]
$$

Unary Operators
$$
\inference{
	\tologic{\env}{e}{\tbool}{p}{\tbool}{\smtenv}{\axioms}
}{
	\tologic{\env}{\lnot e}{\tbool}{\lnot p}{\tbool}{\smtenv}{\axioms}
}[\lgun]
$$
$$
\inference{
	\tologic{\env}{e}{\tbool}{p}{\tbool}{\smtenv}{\axioms}
}{
	\tologic{\env}{\odot\ e}{\tbool}{\odot\ p}{\tbool}{\smtenv}{\axioms}
}[\lgun]
$$

Partially applied operators
$$
\inference{
}{
	\tologic{\env}{\odot}{\constty{\odot}}{\text{uvar}_\odot}{\embed{\constty{\odot}}}{\emptyset}{\etrue}  
}[\lgpop]
$$

$$
\inference{
}{
	\tologic{\env}{\dc}{\constty{\dc}}{\dc}{\embed{\constty{\dc}}}{\emptyset}{\etrue}
}[\lgdc]
$$

$$
\inference{
}{
	\tologic{\env}{x}{\env(x)}{x}{\embed{\env(x)}}{\emptyset}{\etrue}
}[\lgvar]
$$

$$
\inference{
 	f \not \in \smtenv & f \not \in \env & 
 	\sort' = \embed{\tfun{x}{\typ_x}{\typ}} & 
 	\sort  = \embed{\typ} & 
 	\sort_x = \embed{\typ_x} \\
 	\tologic{\env,\tbind{x}{\typ_x}}{e}{\typ}{p}{\sort}{\smtenv, \tbind{x}{\embed{\typ_x}}}{\axioms} \\
  	\axioms_{f_1} = \forall \tbind{x}{\sort_x}.\smtappname{\sort_x}{\sort}\ f\ x = p \\
  	\axioms_{f_2} = \forall \tbind{g}{\sort'}. 
  	(\forall \tbind{x}{\sort_x}. \smtappname{\sort_x}{\sort}\ f\ x = \smtappname{\sort_x}{\sort}\ g\ x) \Rightarrow f = g
}{
	\tologic{\env}{(\efun{x}{}{e})}{(\tfun{x}{\typ_x}{\typ})}
	        {f}{\sort'}{\smtenv, \tbind{f}{\sort'}}{\axioms \land \axioms_{f_1} \land \axioms_{f_2}}
}[\lgfun]
$$

$$
\inference{
	\tologic{\env}{e_1}{\tfun{x}{\typ_x}{\typ}}{p_1}{\tsmtfun{\embed{\typ_x}}{\embed{\typ}}}{\smtenv}{\axioms_1} \\
	\tologic{\env}{e_2}{\typ_x}{p_2}{\embed{\typ_x}}{\smtenv}{\axioms_2}
}{
	\tologic{\env}{e_1\ e_2}{\typ}{\smtapp{\embed{\tfun{x}{\typ_x}{\typ}}}{p_1}{p_2}}{\embed{\typ}}{\smtenv}{\axioms_1 \land \axioms_2}
}[\lgapp]
$$


$$
\inference{
	\tologic{\env}{e}{\tbool}{p}{\tbool}{\smtenv}{\axioms}\\
	\tologic{\env}{e_i\subst{x}{e}}{\typ}{p_i}{\embed{\typ}}{\smtenv}{\axioms_i}
}{
	\tologic{\env}{\ecaseexp{x}{e}{\etrue \rightarrow e_1; \efalse \rightarrow e_2}}{\typ}
	 {\eif{p}{p_1}{p_2}}{\embed{\typ}}{\smtenv}{\axioms\land\wedge_i\axioms_i}
}[\lgcaseBool]
$$

$$
\inference{
	\tologic{\env}{e}{\typ_e}{p}{\embed{\typ_e}}{\smtenv}{\axioms}\\
	\tologic{\env}{e_i\subst{\overline{y_i}}{\overline{\selector{\dc_i}{}\ x}}\subst{x}{e}}{\typ}{p_i}{\embed{\typ}}{\smtenv}{\axioms_i}
}{
	\tologic{\env}{\ecase{x}{e}{\dc_i}{\overline{y_i}}{e_i}}{\typ}
	 {\texttt{if}\ \checkdc{\dc_i}\ p\ \texttt{then}\ p_i}{\embed{\typ}}{\smtenv}{\axioms\land\wedge_i\axioms_i}
}[\lgcase]
$$

$$
\inference{
	\tologic{\env}{e}{\typ}{p}{\embed{\typ}}{\smtenv}{\axioms}
}{
	\tologic{\env}{e}{\typ}{p}{\embed{\typ}}{\smtenv, \tbind{x}{\sort}}{\axioms}
}[\lgenv]
$$



\begin{lemma}[Type Preservation]
If \tologic{\env}{e}{\typ}{p}{\sort}{\smtenv}{\axioms}, 
then $\sort = \embed{\typ}$.
\end{lemma}


\begin{lemma}[Well Formedness]
If \tologic{\env}{e}{\typ}{p}{\sort}{\smtenv}{\axioms}, 
then \smthastype{\smtenv_I, \embed{\env}, \smtenv}{p}{\embed{\typ}}
and \smthastype{\smtenv_I, \embed{\env}, \smtenv}{\axioms}{\tbool}.
\end{lemma}

% \newcommand\bot{\ensuremath{\perp}}

\begin{theorem}\label{thm:embedding}
If \hastype{\env}{e}{\tbool^{\downarrow}} and 
\tologic{\env}{e}{\tbool}{p}{\tbool}{\smtenv}{\axioms}, 
then 
$\forall \vsub\in\interp{\env}$
there always exists an extension $\embed{\vsub} \subseteq\sigma$ such that
$\sigma \models \axioms$ and 
%% axioms are local 
%
$\evalsto{\applysub{\vsub}{p}}{\etrue}$ $\iff$ $\sigma \models p$.
\end{theorem}


\begin{align*}
\embedexpr{\env} \defeq
  \bigwedge\{ \axioms \land p \mid \tbind{x}{\tref{v}{\btyp^{\downarrow}}{e}} \in \env
   \land \tologic{\env}{e\subst{v}{x}}{\btyp}{p}{\embed{\btyp}}{\smtenv_i}{\axioms}  
   \}
\end{align*}




$$
\inference{
  \tologic{\env}{e_i}{\tbool}{p_i}{\tbool}{\smtenv_i}{\axioms_i}
}{
\embedexpr{\env \Rightarrow e_1 \Rightarrow e_2 } \defeq
  \embedexpr{\env} \land \axioms_1 \land \axioms_2 \Rightarrow p_1 \Rightarrow p_2 
}
$$


\begin{theorem}
If \aissubtype{\env}{\tref{v}{\btyp}{e_1}}{\tref{v}{\btyp}{e_2}} 
then \issubtype{\env}{\tref{v}{\btyp}{e_1}}{\tref{v}{\btyp}{e_2}}
\end{theorem}
\begin{proof}
We fix a $\sub\in\interp{\env}$.
Then forall $(\tbind{x_i}{\tref{v}{\btyp^{\downarrow}}{e_i}}) \in \env$ 
$\evalsto{\applysub{\sub}{e_i\subst{v}{x_i}}}{\etrue}$
 
Then need to show that for each $e$, 
if $e \in \interp{\applysub{\sub}{\tref{v}{\btyp}{e_1}}}$,
then $e \in \interp{\applysub{\sub}{\tref{v}{\btyp}{e_2}}}$.

If $e$ diverges then the statement trivially holds. 
Assume $\evalsto{e}{w}$. 
We need to show that 
If $\evalsto{\applysub{\sub}{e_1\subst{v}{w}}}{\etrue}$ then $\evalsto{\applysub{\sub}{e_2\subst{v}{w}}}{\etrue}$.

Let \vsub the lifted substitution that satisfies the above. 
Then there is an extension $\sigma$, such that 
$\sigma \models \beta_i$, $\sigma \models \alpha_i$, $\sigma\models p_i$, and $\sigma\models q_1$
for 
$\tologic{\env}{e_i\subst{v}{x_i}}{\btyp}{p_i}{\embed{\btyp}}{\smtenv_i}{\axioms_i}$
$\tologic{\env}{e_i\subst{v}{w}}{\btyp}{q_i}{\embed{\btyp}}{\smtenv_i}{\beta_i}$.
%
Since \aissubtype{\env}{\tref{v}{\btyp}{e_1}}{\tref{v}{\btyp}{e_2}} we get 
$$
\bigwedge_i (\axioms_i \land p_i) 
\land \beta_1 \land \beta_2 
\Rightarrow q_1 \Rightarrow q_2
$$
thus $\sigma\models q_2$.
%
By Theorem~\ref{thm:embedding} we get $\evalsto{\applysub{\sub}{e_2\subst{v}{w}}}{\etrue}$.
\end{proof}


==> evaluation.tex <==
\section{Evaluation}\label{sec:evaluation}


\begin{figure}
\begin{itemize}
\item \S~\ref{subsec:ackermann}: Ackermann Properties (Figure~\ref{fig:ackermann})
\item \S~\ref{subsec:fold}: Folding Properties (@universal@ \& @fusion@)
\item \S~\ref{subsec:class}: Class Laws (Figure~\ref{fig:laws}) for @List@ and @Maybe@
\item \S~\ref{subsec:programs}: Proofs and Programs: (@SAT-solve@ \& @unify@)
\end{itemize}
\caption{Summary of Benchmarks}
\label{fig:summary}
\end{figure}


\subsection{Arithmetic Properties}\label{subsec:ackermann}
\input{ackermann}
We used \libname to prove arithmetic properties.
We proved that the fibonacci function is increasing,
as described in \S~\ref{sec:examples}
and the properties of Ackermann function
from~\citep{ackermann} summarized in
Figure~\ref{fig:ackermann}.
%
This figure provides two alternative definitions
for the Ackermann Function. We proved equivalence
of the definition (Prop 1.) and various arithmetic
relations among them.


\spara{Generalizing Increasing Properties}
Property 3. shows that \ack{n}{x} is increasing on $x$.
We derived property 4. by applying the\\
\hbox{@gen_increasing@} theorem
from \S~\ref{sec:examples} with input function
the partially applied Ackermann Function \ack{n}{\star}.
%
We used the same technique to generalize increasing properties
from 8. to 9. on the partially applied funciton \iack{h}{n}{\star}.
%
Property 5. proves that \ack{n}{x} is increasing on the first argument $n$.
To generalize it to 6. we cannot reuse theorem @gen_increasin@,
since it only applies to the first argument,
and we need to define a variant @gen_increasing2@ that
generalizes increasing property on the first argument.

\spara{Existentials}
Properties 11. and 12. are described in~\citep{ackermann}
to hold for almost every $x$.
%
That is, Property 11. is described as
$\exists x_0. x_0 < x \Rightarrow x + l < \ack{n}{x}$.
%
Refinement types cannot express existentials,
thus expressing the above property is (currently)
not feasible, but the minimum $x$ was easy to retrieve.
Thus, we expressed the above statement by specifying $x_0 = l-2$.

\spara{Constructive Proofs}
Property 12. was proved in~\citep{ackermann} using a constructive proofs.
Specifically, it constructed a ``ladder'' if Ackermann invocations
and bounded \iack{h}{n}{x} and \ack{n}{x} with this ``ladder''.
To follow the steps of the proof, we defined a function @ladder@ that
simulated the proofs construction.

\subsection{Folding Properties}\label{subsec:fold}

Next, we proved properties of list folding,
as encoded in Adga~\citep{agdaequational}.
%
The following type encodes the universal property of foldr
\begin{code}
  foldr_univ
    :: f:(a -> b -> b)
    -> h:(L a -> b)
    -> e:b
    -> ys:L a
    -> base:{h [] == e }
    -> step:(x:a -> xs:[a] ->
            {h (x:xs) == f x (h xs)})
    -> {h ys == foldr f e ys }
\end{code}
The \libname proof term of @foldr_univ@
is similar to the one in Agda.
But, there are two major differences.
First, specifications do not support quantifiers:
universal quantification of @x@ and @xs@ in
the step assumption is encoded as functional arguments.
Second, unlike Agda,
\libname does not support optional arguments,
thus to use @foldr_univ@ the proof arguments
@base@ and @step@ that were implicit arguments in Agda
need to be explicitely provided.
%
For example, the following code calls @foldr_univarsal@ to prove
@foldr_fusion@ by explicitely applying proofs for the base and the step arguments
\begin{code}
  foldr_fusion
   :: h:(b -> c)
   -> f:(a -> b -> b)
   -> g:(a -> c -> c)
   -> e:b
   -> z:[a]
   -> x:a -> y:b
   -> fuse: {h (f x y) == g x (h y)})
   -> {(h.foldr f e) z == foldr g (h e) z}

  foldr_fusion h f g e ys fuse
   = foldr_univ g (h.foldr f e) (h e) ys
       (fuse_base h f e)
       (fuse_step h f e g fuse)
\end{code}

As an example, @fuse_base@ is a function with type
\begin{code}
  fuse_base
   :: h:(b -> c)
   -> f:(a -> b -> b)
   -> e:b
   -> { (h.foldr f e) [] == h e }
\end{code}

\subsection{Class Laws}\label{subsec:class}
\input{classlaws}
We used \libname to prove Monoid, Functor, Applicative and Monad Laws,
as in HERMIT~\citep{Farmer15}, as summarized
in Figure~\ref{fig:laws} for user-defined
List and Maybe data types.
%

The purpose of these proofs is to investigate the proving abilities of \libname.
For this purpose, we defined the appropriate class operators on user defined lists,
instead of using Haskell's predefined class instances.
%
In the near future, we plan to embed these proofs
to check the laws on real Haskell instances,
but this requires some engineering from the \liquidHaskell team.


\spara{Maybe is a Monoid}
The library definition of Monoid instance on @Maybe a@
defines @mappend@ as
\begin{code}
  instance (Monoid a)
           => Monoid (Maybe a) where
    mappend (Just x) (Just y)
      = Just (mappend x y)
    ...
\end{code}
%
Since we define @mappend@ as a Haskell function,
rather than an instance,
we have no way to express the above definition.
Instead we define @mappend@ to return the first non @Nothing@
argument, if any:
\begin{code}
  mappend Nothing x  = x
  mappend (Just x) _ = Just x
\end{code}
and prove that satisfies the associativity property.

\spara{Functor}
%
We proved both functor laws of Figure~\ref{fig:laws}
by induction on the argument $xs$.
%
One limitation of \libname name, is that
we know of no way to derive the partial
applied version of these laws.
%
For instance, even though we can prove
$\efmap\ \eid\ xs \equiv \eid\ xs$
we know of no way to derive
$\efmap\ \eid \equiv \eid$.

\spara{Monad}
Monad Laws refer to $\lambda$-functions,
thus their proof require defunctionalization and
the extensionality axioms to prove.

In all,
most of the proofs are straightforward,
using inductive reasoning in the structure of the data constructors
and rewriting the definitions of axiomatized functions.
%
The proofs are Haskell programs, and before checked by \liquidHaskell
they are checked by GHC for simple type errors.
%
Our experience,
during the proof process was that most of the times,
proofs that went thought vanilla GHC type checking,
were actually correct, \ie they were accepted by \liquidHaskell.

\subsection{Combining Proofs and Programs} \label{subsec:programs}
%
We used \libname to prove correctness of Haskell functions
that we could not previously prove,
namely, a SAT solver, and type unification.

\spara{SAT solver}.
We encoded the SAT solver example of~\citep{Zombie}
A solver is a Haskell function that takes as input a logical
@f:Formula@ and returns an assignment that satisfies @f@,
if one exists.

\begin{code}
  solve :: f:Formula
        -> Maybe {a:Assignment | sat a f }
  solve f = find (`sat` f) (assignments f)

  assignments :: Formula -> [Assignment]

  find :: (a -> Bool) -> [a] -> Maybe a

  axiomatize sat
  sat :: Assignment -> Formula -> Bool
  \end{code}

Function @assignments f@ returns all possible assignments of the formula @f@,
@sat a f@ returns True $\iff$ the assignment @a@ satisfies the formula @f@.
%
Verification of @solve@ follows directly from axiomatization of the Haskell function @sat@.

\spara{Term Unification}
As another example, we verified unification of first order terms,
as presented in~\citep{Sjoberg2015}.

We define the Haskell function @unify t1 t2@ that can
1. diverge, 2. return @Nothing@, or 3. return a substitution @su@ such that
@apply su t1 == apply su t2@:

\begin{code}
  inline eq_subst
  eq_subst su t1 t2
    = apply su t1 == apply su t2

  type EQSubst T1 T2 =
    {su:Subst | eq_subst su T1 T2 }

  unify :: t1:Term -> t2:Term
        -> Maybe (EQSubst t1 t2)
\end{code}
%
Note for the specification we axiomatize the Haskell function @apply@,
but we do not axiomatize @unify@.
Thus the user \textit{needs not prove} that @unify@ terminates, which is a complicate proof.
%
As before, we prove correctness by invoking helper lemmas that
are separately proved.
%
For example to prove the post-condition when unifying a variable
@TVar i@ with any type @t@ that does not contain the variable @i@,
we invoke the theorem @theoremVar t2 i@ that inductively proves the requirement

\begin{code}
  unify (TVar i) t2
    | not (i Set_mem freeVars t2)
    = Just $ [(i, t2)]
           `byTheorem` theoremVar t2 i

  theoremVar
    :: t:Term
    -> i:{Int | not (i Set_mem freeVars t) }
    -> { eq_subst [(i, t)] (TVar i) t }
\end{code}	%% $


==> intro.tex <==
%%\begin{comment}
%%
%%Dependent types: Coq and Adga fully dependent types,
%%
%%Utopia: extends liquidHaskell to fully dependent types while preserving decidable and predictable type cheking.
%%
%%\begin{itemize}
%%\item \textit{Curry–Howard correspondence} into action!
%%Theorems are refinement types, proofs are plain Haskell programs.
%%\item Type directed proofs: if it (Haskell) type checks, your proof is (most probably) correct!
%%\item Type directed proofs: if it (liquid) type checks, your proof is provably correct!
%%\end{itemize}
%%\end{comment}

\section{Intoduction}\label{sec:intro}

Is decidable and predictable dependent
type programming in a general purpose
programming language utopic?
%
Traditional dependent type
languages, like Coq~\citep{coq-book}
and Adga~\citep{agda},
have been extensively used for
program verification, but they
are not typically used for
general-purpose programming
as they disallow key features
like non-termination, exceptions
and IO.
%
Such features are embedded in verification oriented
general purpose languages, such as
Dafny~\citep{dafny} and \fstar~\citep{fstar}
that allow for semi-automated, SMT based verification.
%

Verification in such languages is
unpredictable~\citep{Leino16}.
Programs are represented as a
logical model in the SMT logic,
and verification relies on SMT
heuristics that an instable.
%
In between, \liquidHaskell restricts
specification languages to
decidable logics ensuring
predictable verification in
the general-purpose language
Haskell, in the cost of low
expressiveness in specifications.

We present \libname,
an extension to Liquid Types that allows
interpretation of terminating program functions
while preserving predictable and decidable type checking.
%
The common route~\citep{dafny, fstar, HALO} for program function
interpretation is to explicitly model function's behavior as an SMT axiom.
Axiom instantiation relies on SMT heuristics that are impredictable,
leading to the ``butterfly effect'' where
modification in a part of the program changes the outcome of verification in other part.
%
Instead of creating SMT axioms, \libname captures the behavior of functions
in function's return type.
%
That way, implicit axioms instantiations occur at each function invocation
and are fully controlled by the programmer.

\mypara{Function Axiomatization} into the SMT logic has been
commonly used to model program functions in SMT-based program
verification. As an example, consider the fibonacci function
%
\begin{code}
  -- I am a comment fib :: Int -> Int
  fib n
    | n == 0    = 0
    | n == 1    = 1
    | otherwise = fib (n-1) + fib (n-2)
\end{code}

An interpretation of @fib@ function can be a logical axiom that exactly captures its behavior:
$$
\begin{array}{rll}
\forall n. \fib{n} = &\texttt{if}\ n = 0 & \texttt{then}\ 0\\
& \texttt{else if}\ n = 1 & \texttt{then}\ 1\\
& \texttt{else}\ & \fib{(n-1)} + \fib{(n-2)}\\
\end{array}
$$

\mypara{Instantiation} of such axioms is problematic as can lead to
matching loops and unpredictable bahaviors.
%
Consider that the existence of the term \fib{n}
triggers the above axiom during verification.
Then, the instantiation $x := \fib{n}$ will produce the terms
\fib{(n-1)} and \fib{(n-2)}, which give rise to other possible instantiations.
%
To prevent matching loops a `fuel'' parameter~\citep{Amin2014ComputingWA}
can be used to restrict the numbers of the SMT
unrollings of each function.


\liquidHaskell followed a simpler approach to prevent matching loops
and keep verification decidable.
%
The implementation of recursive functions was not encoded at all in the logic.
%
Worse, program functions were (syntactically) not allowed
to appear in the specifications.

\libname extends \liquidHaskell allowing interpretation of terminating
program functions while preserving predictability in three steps.
%
The user marks with @axiomatize@
the program functions she wants to refer to in the specifications, sat @f@.

Then, \libname will
\begin{enumerate}
\item Create a logical uninterpreted function with the same name @f@.
\item Automatically strengthen the result type of @f@'s to exactly capture @f@'s behavior.
\item Unfold the function's definition once into the logic, at each program function invocation.
\end{enumerate}

As an example, say that the user wants to reason about the fibonacci function.
Since @fib@ is provably terminating, the user can ``axiomatize'' it.
\begin{code}
  axiomatize fib
\end{code}

\mypara{Step 1: Definition of} @fib@ \textbf{\emph{in the logic.}}
Initially, the axiomatization annotation declares an uninterpreted function @fib@ in the logic
\begin{code}
  fib :: Int -> Int
\end{code}
%
The logical @fib@ is not directly connected to the program function @fib@.
As far as the logic is concerned, @fib@ only satisfies the congruence axiom
%
$$\forall n, m. n = m \Rightarrow \fib{n} = \fib{m}$$
%

\mypara{Step 2: Connecting logical and program} @fib@ \textbf{\emph{via liquid types.}}
Liquid types are Haskell types refined with logical predicates.
As an example, we define the Liquid Type that describes natural numbers
as values @v@ that are integers and moreover satisfy the predicate @0<=v@:
\begin{code}
  type Nat = {v:Int | 0 <= v}
\end{code}
%
The user can use the @Nat@ Liquid Type alias to specify that @fib@ maps
natural numbers to natural numbers
\begin{code}
  fib :: Nat -> Nat
\end{code}
%
Axiomatization of @fib@  \textit{automatically} strengthens the user specified type for @fib@ to
exactly capture @fib@'s behavior via the homonymous uninterpreted function:
\begin{code}
  fib :: n:Nat
      -> {v:Nat |
          v == if n == 0 then 0
               else if n == 1 then 1
               else fib (n-1) + fib (n-2)
          }
\end{code}
%
With this type each invocation of the program @fib@ function automatically
unfolds the @fib@ definition \textit{once} in the logic.

\mypara{Step 3: Function invocation as logical unfolding.}
When the user invokes @fib@ with, say @0@, in @v == fib 0@,
it can be verified that both @v == fib 0@ and @v == 0@.
Thus, the @fib@ function is unfolded once in the logic concluding that
$\fib{0} = 0$.

As an example, by invoking @fib@ on both @2@, @1@ and @0@, we can verify
that @fib 2 == 1@
\begin{code}
  fib2_safe :: {fib 2 == 1}
  fib2_safe = fib 2 == fib 1 + fib 0
\end{code}
Where we use @{p}@ $\defeq$ @{v:t | p}@ when @t@ is obvious from the context
and @v@ does not appear on @p@.

Note that verification on @safe@ relies on the invocations of @fib@
but not on the way these invocations are combined.
%
SMT-based verifies that directly axiomatize program functions do not require such invocations.
For example, \fstar and Dafny can verify the following @fib2@ specification that fails in
\liquidHaskell
%
\begin{code}
  fib2_unsafe :: {fib 2 == 1}
  fib2_unsafe = ()
\end{code}
%
Yet, verification of @fib2_safe@ requires invoking @fib@ on @2@, @1@, and @0@
so that the @fib@ function is unfolded exactly once on these arguments.
%
But, the combination of these function calls in not important.
For example the following term suffices to prove the equality @fib 2 == 2@
\begin{code}
  fib2_safe_tuple :: {fib 2 == 1}
  fib2_safe_tuple = (fib 2, fib 1, fib 0)
\end{code}
%
Even though @fib2_safe@ provides the same information as
@fib2_ safe_tuple@,
it has a better structure regarding the proof it provides.
%
We implemented the library \libname, that smoothly complements the
current extensions in \liquidHaskell, by providing operators that
intuitively structure proofs.

In this paper we present how we extended \liquidHaskell
to allow for arbitrary terminating expressions appear in the specifications.
%
This extension allows the user to specify theorems about program functions
using Liquid Types and prove such theorems using Haskell Code,
instantiating Curry–Howard correspondence.
\begin{itemize}
\item First, we describe the library \libname,
a Haskell library that structures ``axiomatized'' Haskell's functions invocations
into readable, type directed proofs that are checked using \liquidHaskell
(\S~\ref{sec:library}).
%
\item Then, we use \libname to state and prove theorems theorems
on integers (\eg fibonacci function is increasing)
and inductive lists (\eg associativity of append, map fusion, and monad laws)
%
(\S~\ref{sec:examples}).
\item Next, we formalize our system by showing that
the presented extension is sound with respect to denotational semantics
%
(\S~\ref{sec:formalism})
and we present a transformation from a core calculus to
the SMT logic that via lambda lifting and defunctionalization
preserves decidable type checking
of higher order specifications (\S~\ref{sec:algorithmic}).
%
In present of lambda expressions in the specifications,
our translation can (optionally) insert extensionality axioms
that express $\alpha$- and $\beta$-equivalence in the logic,
but do not preserve undecidability and thus unpredictability of type checking.

\item Finally, we evaluated our extension by verification of
arithmetic properties of the Ackermann functions,
class laws on inductive data types,
folding properties,
and by combining proof terms on (potentially diverging)
Haskell programs (\S~\ref{sec:evaluation}).
\end{itemize}


==> logicallifting.tex <==
\section{Logical Lifting}

\begin{figure}[t!]
\centering
$$
\begin{array}{rrcl}
\emphbf{Program} \quad 
  & \prog & ::= & e \spmid \elet{x}{e}{\gtyp}{[L]}{\prog}\\
  & & \spmid & \eletrec{x}{e}{\gtyp}{[L]}{\prog}
\\[0.03in] 

\emphbf{Logic Label} \quad 
  & \prog & ::= & A \spmid M \spmid I 
\end{array}
$$
\end{figure}
\subsubsection{Axioms}
Axioms that are instantiated via function calls. 

\newcommand\exacttype[2]{\ensuremath{\mathtt{exact}(#1, #2)}\xspace}
\newcommand\exacttypefun[3]{\ensuremath{\mathtt{exactfun}(#1, #2, #3)}\xspace}
\newcommand\inline[2]{\ensuremath{[#1 := #2]}\xspace}
\begin{align*}
\embed{\eletrecopt{x}{e}{\gtyp}{A}{\prog}}
  &= \eletrecopt{x}{e}{\exacttype{\gtyp}{e}}{}{\embed{\prog}}\\
\embed{\eletrecopt{x}{e}{\gtyp}{\star}{\prog}}
  &= \eletrecopt{x}{e}{\gtyp}{\star}{\embed{\prog}}\\
\embed{e} &= e 
\end{align*}


\begin{align*}
\exacttype{\tref{v}{\btyp}{r}}{e} &= \tref{v}{\btyp}{r \land v = e}\\
\exacttype{\tfun{x}{\typ_x}{\typ}}{\efun{y}{}{e}} &=\tfun{x}{\typ_x}{\exacttype{\typ}{e\subst{y}{x}}} 
\end{align*}


\subsubsection{Inlines}
Non-recursive logical macros. Can be used only to non-recursive functions. 
\NV{We need to explicitly track recursion}

\begin{align*}
\embed{\elet{f}{\efun{\overline{x}}{}{e}}{\gtyp}{I}{\prog}}
  &= \elet{f}{\efun{\overline{x}}{}{e}}{\gtyp}{}{\embed{\prog\inline{f\ \overline{x}}
  {e}}}\\
\embed{\eletrecopt{x}{e}{\gtyp}{\star}{\prog}}
  &= \eletrecopt{x}{e}{\gtyp}{\star}{\embed{\prog}}\\
\embed{e} &= e 
\end{align*}


\begin{align*}
{\eletrecopt{x}{e}{\gtyp}{\star}{\prog}}\inline{f\ \overline{x}}{e_f}\\
  = \eletrecopt{x}{e}{\gtyp\inline{f\ \overline{x}}{e_f}}{\star}{\prog\inline{f\ \overline{x}}{e_f}}\\
e\inline{f\ \overline{x}}{e_f} = e 
\end{align*}


\begin{align*}
(\tfun{x}{\typ_x}{\typ})\inline{f\ \overline{x}}{e_f}
 = & \tfun{x}{\typ_x\inline{f\ \overline{x}}{e_f}}{\typ\inline{f\ \overline{x}}{e_f}}\\
\tref{v}{\btyp}{e}\inline{f\ \overline{x}}{e_f}
 = & \tref{v}{\btyp}{e\inline{f\ \overline{x}}{e_f}}
\end{align*}

\begin{align*}
(x\ \overline{e})\inline{f\ \overline{x}}{e_f} &= e_f\subst{\overline{x}}{\overline{e}}\\
c\inline{f\ \overline{x}}{e_f} &= c \\
(\efun{x}{\typ}{e})\inline{f\ \overline{x}}{e_f} &=  
\efun{x}{\typ}{e\inline{f\ \overline{x}}{e_f}}\\
(D\ \overline{e})\inline{f\ \overline{x}}{e_f} &=  
D\ \overline{e\inline{f\ \overline{x}}{e_f}}\\
x\inline{f\ \overline{x}}{e_f} &= x \\
(e_1 \ e_2)\inline{f\ \overline{x}}{e_f} &=  (e_1\inline{f\ \overline{x}}{e_f})\ (e_2\inline{f\ \overline{x}}{e_f})\\
\ecase{x}{e}{C}{\overline{x}}{e}\inline{f\ \overline{x}}{e_f} &= 
\ecase{x}{e\inline{f\ \overline{x}}{e_f}}{C}{\overline{x}}{e\inline{f\ \overline{x}}{e_f}}
\end{align*}


\newcommand\updatedcty[2]{\ensuremath{\mathtt{updatedc}(#1, #2)}\xspace}

\subsubsection{Measures}
  Axioms that are automatically instantiated, always.
  \NV{can we encode them using axioms?}
  \NV{not efficient as call invocations}

\begin{align*}
\embed{\eletrecopt{x}{e}{\gtyp}{M}{\prog}}
  &= \eletrecopt{x}{e}{\gtyp}{}{\embed{\prog}}
; \updatedcty{x}{e} \\
\embed{\eletrecopt{x}{e}{\gtyp}{\star}{\prog}}
  &= \eletrecopt{x}{e}{\gtyp}{\star}{\embed{\prog}}\\
\embed{e} &= e 
\end{align*}


\begin{align*}
\updatedcty{f}{\efun{x}{\typ}{\ecase{y}{x}{\dc_i}{\overline{z}}{e_i}}}\\
 \defeq 
 \constty(\dc_i) := \exacttypefun{f}{\constty(\dc_i)}{\efun{\overline{z}}{}{e_i\subst{x}{v}\subst{y}{v}}}
\end{align*}

\begin{align*}
\exacttypefun{f}{\tref{v}{\btyp}{r}}{e} &= \tref{v}{\btyp}{r \land f\ v = e}\\
\exacttypefun{f}{\tfun{x}{\typ_x}{\typ}}{\efun{y}{}{e}} &=\tfun{x}{\typ_x}{\exacttype{\typ}{e\subst{y}{x}}} 
\end{align*}


==> scratch.tex <==
%%% \footnote{Anecdotally, with proof-to-code ratios of 6:1
%%% instead of 50:1 or 100:1 with classical proof assistants~\citep{Ironfleet}},

%%% In present of lambda expressions in
%%% the specifications, our translation
%%% can (optionally) insert extensionality
%%% axioms that express $\alpha$- and
%%% $\beta$-equivalence in the logic,
%%% but do not preserve undecidability
%%% and thus unpredictability of type checking.

Structure
* Introduction
* Overview
* Refinement Reflection
* Algorithmic Checking
* Proof Combinator Library
* Evaluation
* Related Work
--------------------------------------------------------------------------------
Dependently typed languages like demonstrate the
immense potential of writing proofs \emph{of}
programs, \emph{by} programs.
%
They enable developers to \emph{specify} correctness
properties and to \emph{verify} those properties, by
writing both the propositions and the proofs as
ordinary terms in the language, thereby uniting
programming and proving into complementary parts
of a whole.
%
Unfortunately, so far, these benefits require one
to work in one of these specially designed languages.
%
Wouldn't it be great to program proofs and write
proofs of programs in \emph{your} favorite language
and libraries, and have them be built and executed
using \emph{your} favorite compilers and run-times?



We used \libname as an assistant
to state and prove theorems
of Haskell functions
on Integers and inductive data types (Lists and Maybe).
%
In this section, we present by examples how \libname
can be used to prove properties on linear arithmetic
(\eg @fib@ is increasing), higher order properties on
integers and inductive data types (\eg generalization
of increasing property and map fusion), and interpretation
of $\lambda$-terms (\eg associativity of monadic bind).

\spara{Proving Strategies.}
%
The proofs reply on four main proving strategies.
We use color notations to make the proofs more readable.
%
\begin{itemize}
\item\textbf{Theorem application.}
We prove
@f op! g ?  thm e1 .. en@
when the theorem @thm x1 ... xn@
is of the form $(\ttf\ \op ! \ \ttg) \subst{\overline{x}}{\overline{e}}$.
\item \textbf{Definition folding.}
Folding the definition of @f e1 ... en == g@ once
proves that
@rf e1 ... e2 ==! g@
(in which case we color @f@ with red).
%
\item \textbf{Definition unfolding.}
Unfolding the definition of @f e1 ... en == g@ once
proves that
@g ==! gf e1 ... e2@
(in which case we color @f@ with green).
\item \textbf{SMT knowledge}
We rely on SMT interpretations to prove
linear arithmetic properties (\eg @1 < 2@)
or $\eta$-reduction (\eg @e = (\x -> e) x@).
\end{itemize}

\subsection{Arithmetic Properties}
%
We start by proving arithmetic properties
of Haskell functions.  @fib_incr@ states
and proves that the @fib@ function
from \S~\ref{sec:intro} is increasing.
%
\begin{code}
  fib_incr :: n:Nat -> {fib n <= fib (n+1)}
  fib_incr n
    | n == 0
    =   rfib 0
    <!  gfib 1
    *** QED
    | n == 1
    =   fib 1
    <=! fib 1 + fib 0
    <=! gfib 2
    *** QED
    | otherwise
    =   rfib n
    ==! fib (n-1) + fib (n-2)
    <=! fib n + fib (n-2) ? fib_incr (n-1)
    <=! fib n + fib (n-1) ? fib_incr (n-2)
    <=! gfib (n+1)
    *** QED
\end{code} %$
Proofs are total and terminating Haskell functions.
@fib_incr@ proves that @fib n@ is increasing using three cases.
1. If @n==0@,
  then by unfolding @fib@ we get @fib 0 == 0@.
  SMT proves that $0 < 1$, which in turn is folded to @1 == fib 1@.
2. If @n==1@, since @fib@ always returns @Nat@, SMT proves that @fib 1 <= fib 1 + fib 0@
 which is folded to @fib 2@.
3. Otherwise,
  @fib n@ is unfolded to @fib n = fib (n-1) + fib (n-2)@.
  We recursively apply the theorem to the (provably) smaller arguments @n-1@ and @n-2@,
  and fold the result to get @fib n + fib (n-1) = fib (n+1)@.

\subsection{Higher Order Theorems}\label{subsec:higherorder}
Next, we state and prove a generalization of increasing functions.
Namely, that for every function @f@,
if there is a proof that @f@ is increasing, that is,
an expressions with type @z:Nat -> {f z <= f (z+1)}@,
then, for every @x:Nat@ and @y@ greater than @x@,
we prove that @f x <= f y@.
%
\begin{code}
  type Greater N = {v:Int | N < v}

  gen_incr :: f:(Nat -> Int)
           -> (z:Nat -> {f z <= f (z+1)})
           -> x:Nat
           -> y:Greater x
           -> {f x <= f y}
           / [y]
  gen_incr f thm x y
    | x + 1 == y
    =   f x
    <=! f (x+1) ? thm x
    <=! f y
    *** QED
    | x + 1 < y
    =   f x
    <=! f (y-1) ? gen_incr f thm x (y-1)
    <=! f y     ? thm (y-1)
    *** QED
\end{code}
%
We prove the theorem by induction on @y@,
which is stated by the termination metric~\citep{Vazou15} @[y]@.
%
If @x+1 == y@, then we apply the @thm@ argument.
Otherwise, @x+1<y@ and the theorem holds by induction on @y@.

We use the above theorem to directly prove
that @fib@ in increasing with the generalized notion:
%
\begin{code}
  fib_incr_gen :: n:Nat
               -> m:Greater n
               -> {fib n <= fib m}
  fib_incr_gen = gen_incr_eq fib fib_incr
\end{code}


\RJ{FIXME, moved from examples}
\subsection{Example: Reflecting Lists} \label{subsec:list}

%
In the rest of this section, we use \libname to prove
properties about a user defined inductive List data type
\begin{code}
  data L [length] a = N | C a (L a)
\end{code}
%
The annotation @[length]@ on the List definition
states that \liquidHaskell will use the @length@ of lists
as a default termination metric on functions inductive on lists.
%
Where @length@ is defined as expected to map lists to natural numbers
\begin{code}
  measure length
  length :: L a -> Nat
  length N        = 0
  length (C _ xs) = 1 + length xs
\end{code}
%
The @measure@ definition (as defined in~\citep{Vazou14})
translates the @length@ function to refinements in the list's
data constructors.
%
Specifically, the above definition strengthens list's data constructors
as
\begin{code}
 N :: {v:L a | length v == 0 }
 C :: x:a -> xs:L a
   -> {v:L a | length v == 1 + length xs }
\end{code}

Moreover, the \liquidHaskell flag @exact-data-constructors@,
automatically generates the
logical record selectors and checkers for lists.
%
Specifically, the following measures will get generated:
\begin{code}
  is_N N          = True
  is_N (C _ _)    = False

  is_C (C _ _)    = True
  is_C N          = False

  sel_C_1 (C x _) = x
  sel_C_2 (C _ x) = x
\end{code}

\subsection{Append Associativity}\label{subsec:append}
Next we recursively define and axiomatize list append
\begin{code}
  axiomatize (++)
  (++) :: L a -> L a -> L a
  N        ++ ys = ys
  (C x xs) ++ ys = C x (xs ++ ys)
\end{code}
%
The above axiomatization, will automatically produce a type for append
that exactly captures its implementation.
%
\begin{code}
  (++) :: xs:L a -> ys:L a ->
    {v:L a |
       v == if (is_N xs) then ys
            else C (sel_C_1 xs)
                   (sel_C_2 xs ++ ys) }
\end{code}
%
The formal translation of arbitrary terminating functions
is formalized in \S~\ref{sec:algorithmic}.

